InfiX-V1: New Progressive Training Paradigm towards Cost-Efficient Frontier Intelligence

We introduce PACE (Progressive Adaptive Cognitive Expansion), a new cost-effective training paradigm that adapts the learning pace to a model's evolving capacity rather than training with a fixed model architecture and data schedule from the start. PACE mitigates late-stage learning slowdown from fixed model capacity through three co-designed pillars. First, InfiGrow incrementally expands model width and depth during pre-training; under matched compute budgets, our Growth Scaling Law experiments show that it consistently outperforms training with a fixed model scale. Second, InfiCoscale co-scales training data diversity, difficulty, and quality in step with each growth stage, avoiding wasted compute on data mismatched to current model capacity. Third, InfiEPFlow provides system-level expert-parallel load balancing scheme that jointly optimizes computation and communication, improving training efficiency by 8% over force balancing while maintaining strict compute balance. Through four successive growth steps under PACE, we train InfiX-V1, a Mixture-of-Experts (MoE) model with 209B total and 14B activated parameters at remarkably low cost. InfiX-V1-base achieves state-of-the-art performance, surpassing DeepSeek-V4-Flash-Base and MiMo-V2.5-Base; following post-training, InfiX-V1-preview outperforms DeepSeek-V4-Flash (0731), and matches DeepSeek-V4.1-Flash (1017) across several domains. Ultimately, InfiX-V1 delivers roughly 8x higher intelligence per compute than the best competing model, demonstrating that frontier capabilities can be achieved far more efficiently on a paced training path.

==> tables/ablation_width_depth.tex <==
\begin{table}[!t]
    \centering
    \caption{
        Depth growth alone vs.\ width growth followed by depth growth, evaluated after 170B training tokens.
        Baseline: the model without growth in \autoref{tab:ablation_upscale}.
        Depth: depth growth by stacking from the baseline in \autoref{tab:ablation_upscale}, with 43 layers, 64 routed experts and 6 activated experts.
        Width-Depth: width growth followed by depth growth, with 43 layers, 128 routed experts and 12 activated experts.
    }
    \label{tab:ablation_width_depth}
    \setlength{\tabcolsep}{1pt}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l c c c c c c c c c @{}}
    \toprule
    \textbf{Model} & MMLU & MMLU-Pro & BBH & CMMLU & GSM8K & MATH & HumanEval & MBPP & Avg. \\
    \midrule
    Baseline & 51.2 & 24.5 & 35.6 & 55.8 & 36.3 & 15.2 & 17.7 & 31.9 & 33.5 \\
    Depth & 57.3 & 29.0 & 43.6 & 60.6 & 44.7 & 19.5 & 22.6 & 39.3 & 39.6 \\
    Width-Depth & 57.2 & 29.3 & 42.3 & 60.2 & 48.5 & 21.3 & 24.4 & 40.5 & 40.5 \\
    \bottomrule
    \end{tabular*}
\end{table}

